Sato: Contextual Semantic Type Detection in Tables

Detecting the semantic types of data columns in relational tables is important for various data preparation and information retrieval tasks such as data cleaning, schema matching, data discovery, and semantic search. However, existing detection approaches either perform poorly with dirty data, support only a limited number of semantic types, fail to incorporate the table context of columns or rely on large sample sizes for training data. We introduce Sato, a hybrid machine learning model to automatically detect the semantic types of columns in tables, exploiting the signals from the context as well as the column values. Sato combines a deep learning model trained on a large-scale table corpus with topic modeling and structured prediction to achieve support-weighted and macro average F1 scores of 0.925 and 0.735, respectively, exceeding the state-of-the-art performance by a significant margin. We extensively analyze the overall and per-type performance of Sato, discussing how individual modeling components, as well as feature categories, contribute to its performance.

==> background.tex <==
\section{Background\label{sec:background}}
The \sato architecture utilizes three basic machine learning models for automated semantic typing. It builds on a multi-input deep neural network that takes a data feature vector characterizing the data values of a given table column and a topic vector representing the {\em intent} of the table. \sato uses a latent Dirichlet allocation (LDA)~\cite{Blei:2003:LDA} model to represent the intent of a given table through a vector of probabilities corresponding to topics that might be present in the table. \sato then uses a linear-chain conditional random field (CRF)~\cite{Lafferty:2001:CRF} to learn a joint distribution of semantic types, combining the output of the neural network model for each column.  In the following, we provide the minimum required background on these models to help readers follow the rest of the paper. 

% \begin{}
\subsubsection{Deep Learning}
\madelon{Is this detailed explanation necessary?}
Deep learning~\cite{LeCun:2015:DeepLearning} is a form of representation learning that uses neural networks with multiple layers. Through simple but non-linear transformations of the input representation at each layer, deep learning models can learn representations of the data at varying levels of abstractions that are useful for the problem at hand (e.g., classification, regression). Provided enough training data and compute power, neural networks with multiple layers can be effectively trained with a stochastic gradient descent, where the gradient of an objective function with respect to the layer-wise transformation coefficients (i.e., weights)  can be computed using the backpropagation algorithm~\cite{rumelhart1986learning}. The backpropagation procedure is basically an application of the chain rule to compute the derivative of the objective function with respect to the weights in the model by working backwards from the output layer to the input layer, computing the derivative of the output of a unit at each layer with respect to the input of the unit from the preceding layer.  With the increased availability of large-scale training data and compute power, deep learning models showed remarkable improvement and practical success in solving long lasting problems in machine learning, ranging from image recognition to language translation in the last decade. 

Deep learning combined with the availability of massive table corpora~\cite{hu2019viznet,webtables} also presents opportunities to learn from tables in the wild~\cite{halevy2009unreasonable} and improve existing approaches on semantic type detection as well as other research problems around data preparation and information retrieval.  Although prior research used shallow neural networks in the past for related tasks (e.g.,~\cite{li1994semantic}),  only very recently Hulsebos et al.~\cite{Hulsebos:2019:KDD} developed a large-scale deep learning model for semantic typing, achieving state-of-the-art results. 

% Deep Learning~\cite{LeCun:2015:DeepLearning} is a group of machine learning methods that use neural networks with multiple layers. 
% % We can train neural network models in the same manner as other supervised machine learning methods.
% % Feature
% Like other machine learning models, deep learning models are flexible with the input features. It is also common to combine multiple sub-networks to construct a single deep learning model. 
% %
% Single column prediction: (Will copy section here)
% Existing research such as Sherlock~\cite{Hulsebos:2019:KDD} has developed a Deep Learning method for semantic type detection. Sherlock extracts multiple features such word embeddings and global statics from a single column to predict the semantic type. Since the problem is to identify the semantic type of a target column from predefined semantic types, the semantic type detection task can be formulated as a {\it multi-class classification} problem. 
%
% How to use multi-class classification
% For multi-class classification, we design a model to have the same number of output nodes as the classes and use a loss function (e.g., cross-entropy loss) to update the parameters so that the output values get close to training signals in terms of the loss values. 

% Benefit
% The main benefit of deep learning models is the ability to learn representations from data. It is known that trained deeper layers of a deep learning model combine signals to derive semantic representations~\cite{LeCun:2015:DeepLearning}. 


% If we look at a table, a column consists of cells with each carrying a few words. \yoshi{What about numeric values?} We then can aggregate all words and represent this column by a word collection. We can usually separate two columns by their word collections. For example, we may have two collections such as ``Florence, Warsaw, London, ...'' and ``1820-05-12, 1867-11-07, 1912-06-23, ...''. Assume there are two types, i.e. ``city'' and ``date'', we can easily assign type ``city'' to the former collection and type ``date'' to the latter one. We give such assignment because we see a difference in the vocabulary used and such difference is enough to differentiate two columns. When we embed word collection into a vector (e.g., bag-of-words) and feed vectors into a machine model such as Logistic Regression, we are able to learn a classifier that predicts the type of a column based on the vocabulary.

\subsubsection{Topic Models}
Finding topical composition of textual data is useful for many tasks from summarization to featurization of documents. Topic models~\cite{Blei:2012:TopicModels} aim to automatically discover thematic topics in text corpora and discrete data collections in an unsupervised manner.  Latent Dirichlet allocation (LDA)~\cite{Blei:2003:LDA} is a simple yet powerful generative probabilistic topic model, widely used for quantifying thematic structures in text. LDA represents documents as random mixtures of latent topics and each latent topic as a distribution over words.  The main advantage of probabilistic topic models such as LDA  over clustering algorithms is that probabilistic topic models can represent a data point (e.g., document) with a mixture of topics. In other words, probabilistic models provide {\em soft} cluster (topic) membership assignment for each data point (e.g., [0.2, 0.3, 0.5] for three topics), in contrast to {\em hard} membership assignments of standard clustering algorithms such as K-means. Therefore, LDA can also be considered a dimensionality reduction or embedding algorithm for discrete data. Although LDA was originally applied to text corpora, many variants have been developed since then to discover thematic structures in non-textual data as well (e.g.,~\cite{Yuan:2012:DRD, fei2005bayesian,blei2003modeling}).


% Finding semantic topical composition of textual data is useful for many tasks from summarization to featurization.   
% Topic models~\cite{Blei:2012:TopicModels} are machine learning models that aim to discover thematic topics in text or discrete data in a fully unsupervised manner.
% Topic modeling algorithms analyze the contents of text corpora, model 
% % are an unsupervised machine learning framework and a powerful tool that enables us to describe a generative process of data so that we can infer latent structures of data, without any label information. 
% We can use topic models for not only clustering but also extract a topic distribution of each sample to understand the insights of data deeper than clustering algorithms. The topic distribution can be used as additional features for supervised machine learning models. The main difference and advantage against clustering algorithms are that topic models are capable of modeling a data point is generated by aggregations of multiple latent topics. In other words, topic models provide {\it soft assignments} of clusters to each data point (e.g., (0.2, 0.3, 0.5) for three clusters)  in contrast to {\it hard assignments} of clusters by discrete clustering algorithms such as K-means. 

% Latent Dirichlet allocation (LDA)~\cite{Blei:2003:LDA} is the most popular topic model, which models each document has its own latent topic distribution and the words in the document are ``generated’’ based on the word distributions of each topic. LDA was originally applied to a text corpus, but many variants were developed for modeling non-textual sources including human mobility data~\cite{Yuan:2012:DRD}, \todo{XXXX~\cite{}, and YYYY~\cite{}.}  The main difference and advantage against clustering algorithms are that topic models are capable of modeling a data point is generated by aggregations of multiple latent topics. In other words, topic models provide {\it soft assignments} of clusters to each data point (e.g., (0.2, 0.3, 0.5) for three clusters)  in contrast to {\it hard assignments} of clusters by discrete clustering algorithms such as K-means. 


% Structured output learning~\cite{Lafferty:2001:CRF, Smith:2011:LinguisticStructurePrediction, Nowozin:2011:StructuredLearningCV} is a machine learning framework that directly models structure(s) in prediction. In contrast to conventional machine learning models that predict individual instances independently, structured output learning models can take into account outputs (predictions) of other instances to implement a combination of predictions for multiple instances. The approach has been applied to a wide variety of applications especially in Computer Vision and Natural Language Processing~\cite{Nowozin:2011:StructuredLearningCV,Smith:2011:LinguisticStructurePrediction}. A major example in NLP is a sequential tagging model for named entity extraction tasks. The named entity extraction tasks can be considered a multi-class classification task where a model predicts if a token is the beginning of, inside, or outside an entity. Some entities consist of multiple tokens and it is more natural to take into account how likely the predictions before/after the target token is part of an entity. Therefore, structured output learning models are commonly used for this type of task that has structures in output space, instead of applying a multi-class classification for each token independently. 

% Conditional Random Fields (CRF)~\cite{Lafferty:2001:CRF} is the most standard technique for structured output learning. 
% %
% CRF takes into account the other predictions in the form of features so that it can also learn how much the model should put weights on the other predictions. Since a CRF model considers a set of predictions as a combination, the computational complexity is exponential to the number of classes. Specifically, the brute-force approach needs to evaluate all possible $T \cdot N^{T}$ states, where $T$ is the length of sequences and $N$ is the number of classes.
% %
% For linear-chain CRF models \yoshi{Need to explain what is linear-chain}, we can use the forward-backward algorithm for efficient computation of a cost of $\mathcal{O}(N^2 T)$. For more advanced? CRF models, loopy Belief Propagation~\cite{} is often used for training and prediction.

% CRF was originally developed as a single model, which is nothing to do with neural network models. Huang et al. \cite{Huang:2015:BiLSTMCRF} developed a CRF layer that can be attached to neural network models.
% %
% {\color{blue} CRF is a special form of Markov Random Fields, which models joint probabilities of random variables (i.e., $P(X, Y)$); CRF models conditional probabilities of target values (i.e., $P(Y|X)$), where $X$ and $Y$ denote a feature vector and a target vector respectively.}



% \jinfeng{I like this sentence. I am wondering whether we can move it to the beginning of section 2.3}\yoshi{what should we add? The benefits are (1) unsupervised clustering, and (2) results are interpretable in the form of topic distribution.}

